The CARMENES search for exoplanets around M dwarfs. Guaranteed time observations Data Release 1 (2016-2020)

The CARMENES instrument was conceived to deliver high-accuracy radial velocity (RV) measurements with long-term stability to search for temperate rocky planets around a sample of nearby cool stars. The broad wavelength coverage was designed to provide a range of stellar activity indicators to assess the nature of potential RV signals and to provide valuable spectral information to help characterise the stellar targets. The CARMENES Data Release 1 (DR1) makes public all observations obtained during the CARMENES guaranteed time observations, which ran from 2016 to 2020 and collected 19,633 spectra for a sample of 362 targets. The CARMENES survey target selection was aimed at minimising biases, and about 70% of all known M dwarfs within 10 pc and accessible from Calar Alto were included. The data were pipeline-processed, and high-level data products, including 18,642 precise RVs for 345 targets, were derived. Time series data of spectroscopic activity indicators were also obtained. We discuss the characteristics of the CARMENES data, the statistical properties of the stellar sample, and the spectroscopic measurements. We show examples of the use of CARMENES data and provide a contextual view of the exoplanet population revealed by the survey, including 33 new planets, 17 re-analysed planets, and 26 confirmed planets from transiting candidate follow-up. A subsample of 238 targets was used to derive updated planet occurrence rates, yielding an overall average of 1.44+/-0.20 planets with 1 M_Earth < M sin i < 1000 M_Earth and 1 d < P_orb < 1000 d per star, and indicating that nearly every M dwarf hosts at least one planet. CARMENES data have proven very useful for identifying and measuring planetary companions as well as for additional applications, such as the determination of stellar properties, the characterisation of stellar activity, and the study of exoplanet atmospheres.

==> CARMENES GTO catalogue_for_arXiv/Tab/occurrence_signals.tex <==
J00051+457 & ~ & ~ & no signal \\      
J00067-075 & ~ & ~ & no signal \\      
J00162+198E & ~ & ~ & no signal \\      
J00183+440$^1$ & 40.68 & 0.0912\% &  rotation\\   
J00184+440 &10136.69 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J00286-066 & ~ & ~ & no signal \\      
J00389+306 &20.17 & 0.0203\% &  unsolved \\    
J00570+450 & ~ & ~ & no signal \\      
J01013+613 & ~ & ~ & no signal \\      
J01025+716 &43.53 & $ < 10^{-6} $ &  dLW \\    
J01026+623$^1$ & 18.9 & 0.0359\% &   H$\alpha$ \\  
J01026+623$^1$ & 9.35 & 0.0036\% &  rotation \\   
J01048-181 & ~ & ~ & no signal \\      
J01125-169$^1$ &3.06 & 0.0108\%  &  known planet \\   
J01125-169$^1$ &4.7 & 0.0346\%  &  known planet \\   
J01125-169$^1$ &80.77 & 0.0004\% &   dLW \\  
J01339-176 & ~ & ~ & no signal \\      
J01433+043 & ~ & ~ & no signal \\      
J01518+644 & ~ & ~ & no signal \\      
J02002+130 &1.95 & $ < 10^{-6} $ &   H$\alpha$, CRX, dLW \\
J02002+130 &782.52 & $ < 10^{-6} $ &  known planet \\    
J02015+637 & ~ & ~ & no signal \\      
J02070+496 & ~ & ~ & no signal \\      
J02123+035 & ~ & ~ & no signal \\      
J02222+478$^4$ &28.29 & 0.0048\% &   dLW \\  
J02336+249 & ~ & ~ & no signal \\      
J02358+202 & ~ & ~ & no signal \\      
J02362+068 & ~ & ~ & no signal \\      
J02442+255 & ~ & ~ & no signal \\      
J02530+168 &11.41 & $ < 10^{-6} $  &  known planet \\   
J02530+168 &174.09 & $ < 10^{-6} $ &   CRX \\  
J02530+168 &4.91 & $ < 10^{-6} $  &  known planet \\   
J02565+554W & ~ & ~ & no signal \\      
J03133+047 &2.29 & $ < 10^{-6} $  &  known planet \\   
J03133+047 &67.52 & 0.2525\%  &  rotation \\   
J03181+382 & ~ & ~ & no signal \\      
J03213+799 & ~ & ~ & no signal \\      
J03217-066 & ~ & ~ & no signal \\      
J03463+262 & ~ & ~ & no signal \\      
J03531+625 & ~ & ~ & no signal \\      
J04153-076 &1.8 & $ < 10^{-6} $ &   CRX \\  
J04225+105 & ~ & ~ & no signal \\      
J04290+219 &12.54 & 0.0036\% &  rotation \\   
J04290+219 &170.18 & 0.0489\% &  CRX \\    
J04290+219 &24.99 & 0.0326\% &   H$\alpha$, dLW \\ 
J04376-110 & ~ & ~ & no signal \\      
J04376+528 &16.32 & 0.3865\% &   H$\alpha$, dLW \\ 
J04376+528 &419.62 & 0.7739\% &   CaIRT \\  
J04376+528 &7.9 & 0.3618\% &  unsolved \\    
J04429+189$^3$ & ~ & ~ & no signal \\      
J04429+214 & ~ & ~ & no signal \\      
J04520+064$^2$ &10582.5 & 0.1972\% &  $P$ > $\frac{2}{3}$ time baseline \\
J04538-177$^1$ $^3$ & ~ & ~ & no signal \\      
J04588+498 &8.89 & 0.0140\% &  unsolved \\    
J05033-173 &1.92 & 0.0015\% &  candidate \\    
J05033-173 &73.78 & 0.4055\% &  unsolved \\    
J05127+196 & ~ & ~ & no signal \\      
J05280+096 & ~ & ~ & no signal \\      
J05314-036 &1362.47 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J05314-036 &34.09 & 0.0022\% &   H$\alpha$ \\  
J05348+138 & ~ & ~ & no signal \\      
J05360-076 & ~ & ~ & no signal \\      
J05365+113 &11.76 & $ < 10^{-6} $ &   H$\alpha$, dLW \\ 
J05365+113 &12.45 & 0.0043\% &   H$\alpha$, dLW \\ 
J05365+113 &6.31 & 0.0836\% &  activity \\    
J05366+112 & ~ & ~ & no signal \\      
J05415+534 &9.03 & 0.0070\% &   CaIRT \\  
J05421+124 & ~ & ~ & no signal \\      
J06011+595 &44.0 & 0.0268\% &  dLW \\    
J06011+595 &82.97 & 0.0821\% &   dLW \\  
J06024+498 & ~ & ~ & no signal \\      
J06103+821 &409.8 & 0.0081\% &   CaIRT \\  
J06105-218 &2621.33 & 0.0001\% &  $P$ > $\frac{2}{3}$ time baseline \\
J06371+175$^1$ & ~ & ~ & no signal \\      
J06421+035 & ~ & ~ & no signal \\      
J06548+332 &120.37 & $ < 10^{-6} $  &  rotation \\   
J06548+332 &14.24 & $ < 10^{-6} $  &  known planet \\   
J06548+332 &53.65 & 0.0024\%  &  rotation \\   
J06594+193 & ~ & ~ & no signal \\      
J07033+346 & ~ & ~ & no signal \\      
J07044+682 & ~ & ~ & no signal \\      
J07274+052 &19.62 & 0.0813\% &  known planet \\    
J07274+052 &461.91 & $ < 10^{-6} $ &  unsolved \\    
J07274+052 &95.0 & $ < 10^{-6} $ &  rotation \\   
J07287-032 &616.27 & 0.5847\% &  unsolved \\    
J07319+362N &4.78 & 0.6855\% &  unsolved \\    
J07393+021 &29.78 & 0.0121\% &  activity \\    
J07403-174 &6.61 & 0.1475\% &  unsolved \\    
J07582+413 & ~ & ~ & no signal \\      
J08119+087 & ~ & ~ & no signal \\      
J08126-215 & ~ & ~ & no signal \\      
J08161+013 &22.45 & 0.1773\% &  rotation \\   
J08293+039 & ~ & ~ & no signal \\      
J08315+730 & ~ & ~ & no signal \\      
J08358+680 &1.73 & 0.1084\% &  unsolved \\    
J08409-234 &710.89 & $ < 10^{-6} $ &  known planet \\    
J08413+594 &10118.37 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J08413+594 &203.24 & $ < 10^{-6} $  &  known planet \\   
J08413+594 &2204.2 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J08526+283 & ~ & ~ & no signal \\      
J09028+680 & ~ & ~ & no signal \\      
J09143+526 &1210.67 & 0.1987\% &  $P$ > $\frac{2}{3}$ time baseline \\
J09143+526 &16.28 & $ < 10^{-6} $ &   H$\alpha$, dLW \\ 
J09144+526 &16.66 & $ < 10^{-6} $ &   H$\alpha$, dLW \\ 
J09144+526 &24.43 & 0.0003\%  &  known planet \\   
J09144+526 &3971.21 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J09307+003 &294.04 & 0.5392\% &  unsolved \\    
J09360-216$^3$ & ~ & ~ & no signal \\      
J09411+132 & ~ & ~ & no signal \\      
J09423+559 & ~ & ~ & no signal \\      
J09425+700 &677.39 & 0.7290\% &  unsolved \\    
J09428+700 &2.48 & 0.0303\% &   H$\alpha$ \\  
J09447-182 & ~ & ~ & no signal \\      
J09468+760 & ~ & ~ & no signal \\      
J09511-123 & ~ & ~ & no signal \\      
J09561+627$^4$ &18.69 & $ < 10^{-6} $ &   H$\alpha$, dLW \\ 
J10023+480 &3.82 & 0.7102\% &  known planet \\    
J10122-037 &10.66 & 0.0008\% &  rotation \\   
J10122-037 &21.43 & 0.0048\% &   H$\alpha$ \\  
J10167-119 & ~ & ~ & no signal \\      
J10196+198 &2.24 & $ < 10^{-6} $ &   CRX \\  
J10251-102 & ~ & ~ & no signal \\      
J10289+008$^1$ &317.21 & 0.0051\% &  unsolved \\    
J10350-094 & ~ & ~ & no signal \\      
J10482-113 &1.52 & 0.0415\% &   dLW \\  
J10482-113 &2.93 & 0.1639\% &  rotation \\   
J10508+068 & ~ & ~ & no signal \\      
J10564+070$^4$ &2.7 & $ < 10^{-6} $ &   CRX, dLW \\ 
J10584-107 &1.27 & $ < 10^{-6} $ &   CRX \\  
J11000+228 & ~ & ~ & no signal \\      
J11026+219 &13.76 & 0.0030\% &   CRX \\  
J11026+219 &13.93 & 0.2527\% &   CRX \\  
J11033+359 &12.94 & $ < 10^{-6} $  &  known planet \\   
J11033+359 &2017.54 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J11054+435 &1026.37 & 0.0001\% &  $P$ > $\frac{2}{3}$ time baseline \\
J11055+435 & ~ & ~ & no signal \\      
J11110+304W & ~ & ~ & no signal \\      
J11126+189 & ~ & ~ & no signal \\      
J11306-080 & ~ & ~ & no signal \\      
J11417+427 &45.9 & $ < 10^{-6} $  &  known planet \\   
J11417+427 &639.31 & $ < 10^{-6} $ &   H$\alpha$ \\  
J11417+427 &835.19 & 0.0736\% &  $P$ > $\frac{2}{3}$ time baseline \\
J11421+267 &2.64 & $ < 10^{-6} $  &  known planet \\   
J11467-140 & ~ & ~ & no signal \\      
J11476+786 & ~ & ~ & no signal \\      
J11477+008$^1$ & ~ & ~ & no signal \\      
J11509+483 &316.73 & $ < 10^{-6} $ &  rotation \\   
J11511+352 &11.12 & 0.0014\% &  rotation \\   
J12100-150 & ~ & ~ & no signal \\      
J12111-199 & ~ & ~ & no signal \\      
J12123+544S &13.67 & $ < 10^{-6} $  &  known planet \\   
J12230+640 &15.13 & 0.0005\% &   CRX \\  
J12230+640 &73.06 & 0.0586\% &   CRX \\  
J12230+640 &8254.83 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J12248-182 & ~ & ~ & no signal \\      
J12312+086 & ~ & ~ & no signal \\      
J12373-208 & ~ & ~ & no signal \\      
J12479+097 &1.42 & $ < 10^{-6} $  &  known planet \\   
J12479+097 &650.94 & 0.3179\%  &  unsolved \\   
J13102+477 & ~ & ~ & no signal \\      
J13209+342 &5962.88 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J13229+244 &3.02 & $ < 10^{-6} $  &  known planet \\   
J13229+244 &87.79 & 0.0015\% &   H$\alpha$, CRX, dLW \\
J13299+102$^1$ &15.42 & 0.3861\% &  rotation \\   
J13299+102$^1$ &15.83 & 0.0023\% &  rotation \\   
J13299+102$^1$ &512.48 & 0.0589\% &  unsolved \\    
J13427+332 & ~ & ~ & no signal \\      
J13450+176 & ~ & ~ & no signal \\      
J13457+148 &105.98 & 0.0074\% &  rotation \\   
J13457+148 &306.51 & 0.0020\% &  unsolved \\    
J13457+148 &33.89 & 0.0007\% &  unsolved \\    
J13458-179 & ~ & ~ & no signal \\      
J13582+125 & ~ & ~ & no signal \\      
J14010-026$^3$ & ~ & ~ & no signal \\      
J14082+805 & ~ & ~ & no signal \\      
J14251+518 & ~ & ~ & no signal \\      
J14257+236E & ~ & ~ & no signal \\      
J14257+236W &10002.44 & 0.2462\% &  $P$ > $\frac{2}{3}$ time baseline \\
J14307-086 &252.02 & 0.2434\% &  unsolved \\    
J14342-125 &113.37 & $ < 10^{-6} $ &   CaIRT \\  
J14342-125 &36.11 & 0.0015\% &  known planet \\    
J14524+123 &26.71 & 0.0010\% &  rotation? \\    
J14544+355 & ~ & ~ & no signal \\      
J15013+055 & ~ & ~ & no signal \\      
J15095+031 & ~ & ~ & no signal \\      
J15194-077 &12.92 & 0.0148\%  &  known planet \\   
J15194-077 &5.37 & $ < 10^{-6} $  &  known planet \\   
J15598-082 & ~ & ~ & no signal \\      
J16028+205 & ~ & ~ & no signal \\      
J16167+672N &42.22 & 0.0208\% &  activity \\    
J16167+672S &21.99 & 0.0641\% &   rotation \\  
J16167+672S &365.13 & $ < 10^{-6} $ &   CaIRT, CRX \\ 
J16167+672S &86.43 & $ < 10^{-6} $ &   known planet \\  
J16254+543$^1$ & ~ & ~ & no signal \\      
J16303-126 &1.26 & 0.3514\% &   known planet \\  
J16303-126 &17.88 & $ < 10^{-6} $  &  known planet \\   
J16303-126 &1.84 & 0.3134\%  &  unsolved \\   
J16327+126 & ~ & ~ & no signal \\      
J16462+164 & ~ & ~ & no signal \\      
J16554-083N & ~ & ~ & no signal \\      
J16581+257 &12.42 & 0.0500\% &  rotation \\   
J16581+257$^3$ &661.35 & 0.0033\% &  $P$ > $\frac{2}{3}$ time baseline \\
J17033+514 &6.94 & 0.0752\% &  candidate \\    
J17052-050 & ~ & ~ & no signal \\      
J17071+215 & ~ & ~ & no signal \\      
J17115+384 &5.58 & 0.8902\% &  unsolved \\    
J17166+080 & ~ & ~ & no signal \\      
J17198+417 &23.13 & 0.3605\% &  unsolved \\    
J17303+055 & ~ & ~ & no signal \\      
J17355+616$^3$ & ~ & ~ & no signal \\      
J17364+683 &38.56 & $ < 10^{-6} $ &   known planet \\  
J17378+185 &15.52 & 0.0001\%  &  known planet \\   
J17378+185 &40.28 & 0.4268\% &   H$\alpha$, dLW \\ 
J17378+185 &499.08 & 0.0479\%  &  known planet \\   
J17542+073 &1.55 & 0.2591\% &  activity \\    
J17578+046$^1$ &287.23 & 0.0056\% &  rotation \\   
J17578+046$^1$ &387.44 & 0.2243\% &   CaIRT, H$\alpha$, dLW \\
J17578+046$^1$ &652.12 & 0.0225\% &  unsolved \\    
J17578+465 & ~ & ~ & no signal \\      
J18027+375 & ~ & ~ & no signal \\      
J18051-030 & ~ & ~ & no signal \\      
J18075-159 & ~ & ~ & no signal \\      
J18165+048 &23239.74 & 0.0095\% &  $P$ > $\frac{2}{3}$ time baseline \\
J18174+483 &16.04 & 0.0332\% &  activity \\    
J18174+483 &7.96 & 0.4972\% &   CRX \\  
J18180+387E & ~ & ~ & no signal \\      
J18221+063 & ~ & ~ & no signal \\      
J18224+620 &2.06 & 0.7429\% &   CaIRT \\  
J18319+406 &2.93 & 0.2034\% &  unsolved \\    
J18346+401 &5786.99 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J18353+457$^3$ &2.62 & 0.0842\% &   H$\alpha$ \\  
J18363+136 &8189.81 & 0.9454\% &  $P$ > $\frac{2}{3}$ time baseline \\
J18409-133 &5.1 & 0.2652\% &  candidate \\    
J18419+318 & ~ & ~ & no signal \\      
J18427+596N &11.2 & 0.0018\% &  unsolved \\    
J18427+596N &27647.04 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J18427+596N &64.8 & 0.0871\% &  unsolved \\    
J18427+596S &10000.0 & $ < 10^{-6} $ &  unsolved \\    
J18427+596S &117.9 & 0.0053\% &  unsolved \\    
J18427+596S &186.6 & 0.0209\% &  unsolved \\    
J18480-145 & ~ & ~ & no signal \\      
J18482+076 &1.4 & 0.8063\% &  rotation \\   
J18498-238 &1.43 & 0.0294\% &   CRX, dLW \\ 
J18498-238 &2.89 & $ < 10^{-6} $ &   dLW \\  
J18580+059$^3$ & ~ & ~ & no signal \\      
J19070+208 & ~ & ~ & no signal \\      
J19072+208 & ~ & ~ & no signal \\      
J19084+322 & ~ & ~ & no signal \\      
J19098+176 & ~ & ~ & no signal \\      
J19169+051N$^5$ &132.39 & $ < 10^{-6} $ &   CRX \\  
J19216+208 & ~ & ~ & no signal \\      
J19251+283 & ~ & ~ & no signal \\      
J19346+045 &2.52 & 0.6353\% &  unsolved \\    
J20260+585 &16.21 & 0.0080\% &  known planet \\  
J20260+585 &14.95 & 0.5846\% &  unsolved \\    
J20260+585 &403.71 & $ < 10^{-6} $ &  tellurics \\    
J20305+654 & ~ & ~ & no signal \\      
J20336+617 &175.74 & 0.6727\% &   CRX \\  
J20405+154 &153.66 & 0.7230\% &  unsolved \\    
J20450+444 & ~ & ~ & no signal \\      
J20525-169 & ~ & ~ & no signal \\      
J20533+621 &118.6 & 0.7191\% &   CaIRT, CRX \\ 
J20556-140S & ~ & ~ & no signal \\      
J20567-104 &1.25 & 0.1960\% &  unsolved \\    
J21019-063 & ~ & ~ & no signal \\      
J21152+257 & ~ & ~ & no signal \\      
J21164+025 &14.46 & $ < 10^{-6} $  &  known planet \\   
J21164+025 &43.71 & 0.0006\% &   H$\alpha$ \\  
J21221+229 &39.91 & 0.0001\% &   H$\alpha$, dLW \\ 
J21221+229 &686.81 & $ < 10^{-6} $ &  known planet \\    
J21348+515 &26.33 & 0.7167\% &  rotation \\   
J21463+382 & ~ & ~ & no signal \\      
J21466-001 & ~ & ~ & no signal \\      
J21466+668 &2.31 & $ < 10^{-6} $  &  known planet \\   
J21466+668 &8.05 & 0.0001\%  &  known planet \\   
J21466+668 &92.49 & $ < 10^{-6} $  &  rotation \\   
J22021+014 &10.95 & 0.0373\% &   H$\alpha$ \\  
J22057+656 &122.52 & $ < 10^{-6} $ &   CRX \\  
J22096-046$^2$ &3998.46 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J22114+409 &15.22 & 0.5957\% &  rotation \\   
J22115+184 &374.96 & $ < 10^{-6} $ &   CRX \\  
J22115+184 &39.02 & 0.0015\% &   dLW \\  
J22125+085 &2911.44 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J22137-176 &3.65 & $ < 10^{-6} $  &  known planet \\   
J22137-176 &588.11 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J22231-176 & ~ & ~ & no signal \\      
J22252+594 &13.35 & $ < 10^{-6} $  &  known planet \\   
J22298+414 &5.78 & 0.0280\% &   dLW \\  
J22330+093 &34.06 & 0.6282\% &  unsolved \\    
J22503-070 & ~ & ~ & no signal \\      
J22532-142 &30.07 & $ < 10^{-6} $  &  known planet \\   
J22532-142 &60.85 & $ < 10^{-6} $  &  known planet \\   
J22559+178 & ~ & ~ & no signal \\      
J22565+165 &18.61 & $ < 10^{-6} $ &  rotation \\   
J22565+165 &1845.72 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J22565+165 &39.28 & $ < 10^{-6} $ &   H$\alpha$, dLW \\ 
J23216+172 & ~ & ~ & no signal \\      
J23245+578 & ~ & ~ & no signal \\      
J23340+001 & ~ & ~ & no signal \\      
J23351-023 & ~ & ~ & no signal \\      
J23381-162 & ~ & ~ & no signal \\      
J23419+441 &175.09 & 0.0001\% &  unsolved \\    
J23431+365 & ~ & ~ & no signal \\      
J23492+024 &372.77 & 0.0001\% &   CaIRT \\  
J23492+024 &53.83 & 0.4878\% &   H$\alpha$ \\  
J23505-095 & ~ & ~ & no signal \\  

==> CARMENES GTO catalogue_for_arXiv/Tab/planets_in_sample.tex <==
J00067$-$075 & GJ 1002                &  86 &  53 & $0.120$         & b & $1.31\pm0.14$           & $1.08\pm0.13$          & $10.3465\pm0.0025$                & d & SM22 \\
             &                        &     &     &                 & c & $1.30\pm0.14$           & $1.36\pm0.17$          & $21.202\pm0.013$                  & d & SM22 \\
\noalign{\smallskip}
J00183+440   & GJ 15 A                & 208 & 297 & $0.391\pm0.016$ & b & $1.79\pm0.24$           & $3.98^{+0.38}_{-0.29}$ & $11.436\pm0.001$                  & r & Tri22 \\
             &                        &     &     &                 & c & $1.62^{+0.57}_{-0.36}$  & $50.4^{+6.9}_{-6.8}$   & $6694^{+164}_{-285}$              & d & Tri22 \\
\noalign{\smallskip}
J00403+612   & 2MJ00402129+6112490    &  44 &   0 & $0.471\pm0.011$ & b & $5.83^{+0.86}_{-0.91}$  & $7.52^{+1.12}_{-1.18}$ & $2.527113\pm0.000009$             & f & GA22b \\
             &                        &     &     &                 & c & $3.19^{+1.16}_{-1.07}$  & $7.94^{+2.88}_{-2.64}$ & $18.0881\pm0.0002$                & f & GA22b \\
\noalign{\smallskip}
J01026+623   & GJ 49                  &  80 & 158 & $0.515\pm0.019$ & b & $2.52^{+0.31}_{-0.30}$  & $5.63^{+0.67}_{-0.68}$ & $13.8508^{+0.0053}_{-0.0051}$     & d & Per19 \\
\noalign{\smallskip}
J01066+192   & LSPM J0106+1913        &  65 &  32 & $0.344\pm0.005$ & b & $3.40^{+0.25}_{-0.24}$  & $3.21\pm0.24$          & $1.8805136\pm0.0000025$           & f & Cha22 \\  
             &                        &     &     &                 & c & $3.48^{+0.34}_{-0.35}$  & $6.64^{+0.67}_{-0.68}$ & $15.532482\pm0.000034$            & f & Cha22 \\    
\noalign{\smallskip}
J01125$-$169 & YZ Cet                 & 108 & 332 & $0.142\pm0.010$ & b & $1.31^{+0.15}_{-0.14}$  & $0.70^{+0.09}_{-0.08}$ & $2.02087^{+0.00007}_{-0.00009}$   & r & Sto20a \\ 
             &                        &     &     &                 & c & $1.84^{+0.14}_{-0.15}$  & $1.14^{+0.11}_{-0.10}$ & $3.0599\pm0.0001$                 & r & Sto20a \\ 
             &                        &     &     &                 & d & $1.54^{+0.14}_{-0.15}$  & $1.09\pm0.12$          & $4.65626^{+0.00028}_{-0.00029}$   & r & Sto20a \\ 
\noalign{\smallskip}
J02002+130   & TZ Ari                 &  93 &  79 & $0.150\pm0.010$ & b & $18.8^{+1.3}_{-1.2}$    & $67\pm6$               & $771.4^{+1.3}_{-1.2}$             & d & Qui22 \\
\noalign{\smallskip}
J02489$-$145W& PMJ02489$-$1432W       &  33 &   0 & $0.512\pm0.020$ & b & $4.65^{+0.60}_{-0.64}$  & $6.28^{+0.84}_{-0.88}$ & $2.491986\pm0.000003$             & f & Kos21 \\
\noalign{\smallskip}
J02530+168   & Teegarden's Star       & 238 &   0 & $0.089\pm0.009$ & b & $2.02^{+0.19}_{-0.20}$  & $1.05^{+0.13}_{-0.12}$ & $4.9100\pm0.0014$                 & d & Zec19 \\ %Releasing 252 obs
             &                        &     &     &                 & c & $1.61\pm0.19$           & $1.11^{+0.16}_{-0.15}$ & $11.409\pm0.009$                  & d & Zec19 \\ %Releasing 252 obs
\noalign{\smallskip}
J02573+765   & LHS 1478               &  57 &  13 & $0.236\pm0.012$ & b & $3.13^{+0.23}_{-0.25}$  & $2.33\pm0.20$          & $1.949538\pm0.000004$             & f & Sot21 \\
\noalign{\smallskip}
J03133+047   & CD Cet                 & 106 &   0 & $0.161\pm0.010$ & b & $6.51^{+0.22}_{-0.23}$  & $3.95^{+0.42}_{-0.43}$ & $2.29070\pm0.00012$               & d & Bau20 \\ 
\noalign{\smallskip}
J04167$-$120 & LP714-47               &  34 &  54 & $0.59\pm0.02$   & b & $17.6\pm0.8$            & $30.8\pm1.5$           & $4.052037\pm0.000004$             & f & Dre20 \\
\noalign{\smallskip}
J04343+430   & 2MJ04342248+4302148    &  55 &   0 & $0.495\pm0.019$ & b & $4.41\pm0.73$           & $3.76\pm0.63$          & $0.669140^{+0.000002}_{-0.000002}$& f & Blu21 \\
             &                        &     &     &                 & c & $4.53^{+1.01}_{-1.02}$  & $9.2\pm2.1$            & $9.025^{+0.104}_{-0.119}$         & f & Blu21 \\
\noalign{\smallskip}
J04429+189   & GJ 176                 &  23 & 181 & $0.504\pm0.013$ & b & $4.49^{+1.00}_{-0.23}$  & $9.1^{+1.5}_{-0.7}$    & $8.776^{+0.001}_{-0.002}$         & r & Tri18 \\ 
\noalign{\smallskip}
J06371+175   & HD 260655              &  88 &  92 & $0.439\pm0.011$ & b & $1.69\pm0.27$           & $2.14\pm0.34$          & $2.76953\pm0.00003$               & f & Luq22 \\ %Releasing 56 obs
             &                        &     &     &                 & c & $1.92\pm0.30$           & $3.09\pm0.48$          & $5.70588\pm0.00007$               & f & Luq22 \\
\noalign{\smallskip}
J06548+332   & GJ 251                 & 280 &  75 & $0.360\pm0.015$ & b & $2.24\pm0.18$           & $4.27^{+0.37}_{-0.36}$ & $14.2383\pm0.0018$                & d & Sto20b,TW \\ %Releasing 280 obs
\noalign{\smallskip}
J08023+033   & GJ 3473                &  64 &  88 & $0.360\pm0.016$ & b & $2.21\pm0.35$           & $1.86\pm0.30$          & $1.198003\pm0.000002$             & f & Kem20 \\
             &                        &     &     &                 & c & $3.75^{+0.45}_{-0.42}$  & $7.41^{+0.91}_{-0.86}$ & $15.509\pm0.033$                  & f & Kem20 \\
\noalign{\smallskip}
J08413+594   & GJ 3512                & 182 &   0 & $0.123\pm0.009$ & b & $71.23^{+0.32}_{-0.33}$ & $146\pm7$              & $203.13\pm0.05$                   & d & Mor19,TW \\ %Releasing 182 obs
             &                        &     &     &                 & c & $27.9\pm0.4$            & $143\pm7$              & $2350^{+100}_{-80}$               & d & Mor19,TW \\ %Releasing 182 obs
\noalign{\smallskip}
J09144+526   & GJ 338 B               & 159 &  30 & $0.64\pm0.07$   & b & $3.07\pm0.37$           & $10.27^{+1.47}_{-1.38}$& $24.45\pm0.02$                    & d & GA20 \\
\noalign{\smallskip}
J09360$-$216 & GJ 357                 &  10 & 128 & $0.342\pm0.011$ & b & $1.52\pm0.25$           & $1.84\pm0.31$          & $3.93072^{+0.00008}_{-0.00006}$   & f & Luq19 \\ %Releasing 25 obs
             &                        &     &     &                 & c & $2.13\pm0.28$           & $3.40\pm0.46$          & $9.1247^{+0.0011}_{-0.0010}$      & d & Luq19 \\ %Releasing 25 obs
             &                        &     &     &                 & d & $2.09^{+0.34}_{-0.35}$  & $6.1\pm1.0$            & $55.661\pm0.055$                  & d & Luq19 \\ %%Releasing 25 obs
\noalign{\smallskip}
J10088+692   & TYC4384-1735-1         &  40 &  21 & $0.630\pm0.024$ & b & $3.40^{+0.35}_{-0.34}$  & $5.90^{+0.62}_{-0.61}$ & $3.444717^{+0.000040}_{-0.000042}$& f & Blu20 \\ %Releasing 42 obs
\noalign{\smallskip}
J10185$-$117 & LTT 3780               &  52 &   4 & $0.379\pm0.016$ & b & $3.13^{+0.31}_{-0.3}$   & $2.34^{+0.24}_{-0.23}$ & $0.768377\pm0.000001$             & f & Now20 \\
             &                        &     &     &                 & c & $3.36^{+0.32}_{-0.31}$  & $6.29^{+0.63}_{-0.61}$ & $12.25213^{+0.00007}_{-0.00006}$  & f & Now20 \\
\noalign{\smallskip}
J10289+008   & GJ 393                 &  84 & 250 & $0.426\pm0.017$ & b & $1.01\pm0.14$           & $1.71\pm0.24$          & $7.02679^{+0.00082}_{-0.00085}$   & d & Ama21 \\
\noalign{\smallskip}
J11033+359   & Lalande 21185          & 321 & 416 & $0.390\pm0.011$ & b & $1.39\pm0.14$           & $2.69\pm0.25$          & $12.946\pm0.005$                  & r & Sto20b \\ %Releasing 383 obs
%J11044+304   & LSPM J1104+3027        &     &     &                 & b &                         &                        &                                   & f & ZaOs22 \\
%             &                        &     &     &                 & c &                         &                        &                                   & f & ZaOs22 \\
\noalign{\smallskip}
J11302+076   & K2-18                  &  58 &   0 & $0.359\pm0.047$ & b & $3.38^{+0.76}_{-0.75}$  & $8.49^{+1.97}_{-2.08}$ & $32.9396\pm0.00010$               & f & Sar18 \\ %Releasing 61 obs
\noalign{\smallskip}
J11417+427   & GJ 1148                &  76 & 125 & $0.354\pm0.015$ & b & $38.54^{+0.43}_{-0.37}$ & $96.6^{+1.0}_{-1.3}$   & $41.380^{+0.001}_{-0.002}$        & r & Tri20 \\
             &                        &     &     &                 & c & $12.26^{+0.59}_{-0.56}$ & $72.1^{+3.2}_{-7.0}$   & $532.6^{+1.0}_{-1.1}$             & d & Tri20 \\
\noalign{\smallskip}
J11421+267   & GJ 436                 & 113 & 525 & $0.436\pm0.012$ & b & $17.38\pm0.17$          & $21.36^{+0.20}_{-0.21}$& $2.644^{+0.001}_{-0.001}$         & r & Tri18 \\ %Releasing 124 obs
\noalign{\smallskip}
J11509+483   & GJ 1151                &  97 &  71 & $0.164\pm0.009$ & b & $3.10^{+0.38}_{-0.43}$  & $10.6^{+1.3}_{-1.5}$   & $389.7^{+5.4}_{-6.5}$             & d & Bla22 \\
\noalign{\smallskip}
J12123+544S  & GJ 458 A               & 108 &   0 & $0.578\pm0.021$ & b & $2.85^{+0.38}_{-0.39}$  & $6.89^{+0.92}_{-0.95}$ & $13.671^{+0.011}_{-0.010}$        & d & Sto20b \\
\noalign{\smallskip}
J12479+097   & GJ 486                 &  76 &  65 & $0.323\pm0.015$ & b &$3.370^{+0.078}_{-0.080}$& $2.82^{+0.11}_{-0.12}$ & $1.467119^{+0.000031}_{-0.000030}$& d & Tri21 \\ 
\noalign{\smallskip}
J13229+244   & GJ 3779                & 104 &   0 & $0.27\pm0.02$   & b & $8.62\pm0.39$           & $8.0\pm0.5$            & $3.0232\pm0.0004$                 & d & Luq18 \\ 
\noalign{\smallskip}
J13299+102   & GJ 514                 & 274 & 266 & $0.510\pm0.051$ & b & $1.15^{+0.21}_{-0.19}$  & $5.2\pm0.9$            & $140.43\pm0.41$                   & d & Dam22 \\
\noalign{\smallskip}
J13255+688   & 2MJ13253177+6850106    &  55 &   0 & $0.59\pm0.02$   & b & $3.74^{+1.03}_{-0.99}$  & $3.75^{+1.14}_{-1.06}$ & $0.764597^{+0.000013}_{-0.000011}$& f & GA22a \\ %Releasing 47 obs
             &                        &     &     &                 & c & $5.10^{+1.02}_{-1.06}$  & $8.32^{+1.90}_{-1.88}$ & $3.294736^{+0.000034}_{-0.000036}$& f & GA22a \\ %Releasing 47 obs
\noalign{\smallskip}
J14010$-$026 & GJ 536                 &  28 & 277 & $0.530\pm0.011$ & b & $3.12^{+0.36}_{-0.19}$  & $6.52^{+0.69}_{-0.40}$ & $8.708^{+0.002}_{-0.001}$         & r & Tri18 \\ 
\noalign{\smallskip}
J14342$-$125 & GJ 555                 &  94 &  48 & $0.291\pm0.014$ & b & $5.46\pm0.75$           & $2.59\pm0.34$          & $36.116^{+0.027}_{-0.029}$        & d & GA22c \\
\noalign{\smallskip}
J15194$-$077 & GJ 581                 &  20 & 664 & $0.323\pm0.013$ & b & $12.35^{+0.18}_{-0.20}$ & $15.20^{+0.22}_{-0.27}$& $5.368^{+0.001}_{-0.001}$         & r & Tri18 \\ %Releasing 54 obs
             &                        &     &     &                 & c & $3.28^{+0.22}_{-0.12}$  & $5.65^{+0.39}_{-0.24}$ & $12.919^{+0.003}_{-0.002}$        & r & Tri18 \\ %Releasing 54 obs
             &                        &     &     &                 & e & $1.55^{+0.22}_{-0.13}$  & $1.66^{+0.24}_{-0.16}$ & $3.153^{+0.001}_{-0.006}$         & r & Tri18 \\ %Releasing 54 obs
\noalign{\smallskip}
J15583+354   & GJ 3929                &  73 &   0 & $0.309\pm0.014$ & b & $1.29^{+0.47}_{-0.46}$  & $1.27\pm0.46$          & $2.616267^{+0.000005}_{-0.000005}$& f & Kem22 \\ %Releasing 39 obs
\noalign{\smallskip}
J16167+672S  & HD 147379              & 186 &  30 & $0.58\pm0.08$   & b & $4.87^{+0.41}_{-0.37}$  & $23.0^{+2.8}_{-2.9}$   & $86.57\pm0.06$                    & d & Rei18a,TW \\
\noalign{\smallskip}
J17378+185   & GJ 686                 & 100 & 198 & $0.426\pm0.033$ & b & $3.02^{+0.18}_{-0.20}$  & $6.64^{+0.53}_{-0.54}$ & $15.5314^{+0.0015}_{-0.0014}$     & r & Lal19 \\ 
\noalign{\smallskip}
J17578+046   & Barnard's Star         & 196 & 575 & $0.163\pm0.022$ & b & $1.20\pm0.12$           & $3.23\pm0.44$          & $232.80^{+0.38}_{-0.41}$          & d & Rib18 \\ %Releasing 520 obs
\noalign{\smallskip}
J18580+059   & GJ 740                 &  32 & 129 & $0.58\pm0.06$   & b & $2.13^{+0.34}_{-0.32}$  & $2.96^{+0.50}_{-0.48}$ & $2.37756^{+0.00013}_{-0.00011}$   & d & TP21 \\
\noalign{\smallskip}
J19169+051N  & HD 180617              & 123 & 296 & $0.45\pm0.04$   & b & $2.85^{+0.16}_{-0.25}$  & $12.2^{+1.0}_{-1.4}$   & $105.90^{+0.09}_{-0.10}$          & d & Kam18 \\
\noalign{\smallskip}
J20260+585   & Wolf 1069              & 268 &   0 & $0.167\pm0.011$ & b & $1.07\pm0.17$           & $1.26\pm0.21$          & $15.564\pm0.015$                  & d & Kos22b \\
\noalign{\smallskip}
J20450+444   & GJ 806                 &  67 & 160 & $0.413\pm0.011$ & b & $2.25\pm0.20$           & $1.90\pm0.17$          & $0.9263237\pm0.0000009$           & f & Pal22 \\
             &                        &     &     &                 & c & $3.55\pm0.17$           & $5.80\pm0.30$          & $6.64064\pm0.00025$               & f & Pal22 \\
\noalign{\smallskip}
J20451$-$313 & AU Mic                 & 100 & 310 & $0.50\pm0.03$   & b & $10.23^{+0.88}_{-0.91}$ & $20.12^{+1.72}_{-1.57}$& $8.463000\pm0.000002$             & f & Cal21 \\
             &                        &     &     &                 & c & $<7.7$                  & $<20.1$                & $18.859019\pm0.000016$            & f & Cal21 \\
\noalign{\smallskip}
J21164+025   & LSPM J2116+0234        &  72 &   0 & $0.430\pm0.031$ & b & $6.31^{+0.44}_{-0.43}$  & $13.4\pm1.1$           & $14.4433^{+0.0079}_{-0.0086}$     & d & Lal19 \\ %Releasing 81 obs
\noalign{\smallskip}
J21221+229   & TYC 2187-512-1         &  94 &   0 & $0.498\pm0.019$ & b & $12.02^{+0.47}_{-0.46}$ & $105\pm6$              & $691.9^{+8.8}_{-8.6}$             & d & Qui22 \\
\noalign{\smallskip}
J21466+668   & G264-012               & 159 &   0 & $0.297\pm0.024$ & b & $2.72^{+0.28}_{-0.29}$  & $2.50^{+0.29}_{-0.30}$ & $2.30538\pm0.00031$               & d & Ama21 \\ 
             &                        &     &     &                 & c & $2.69^{+0.31}_{-0.30}$  & $3.75^{+0.48}_{-0.47}$ & $8.0518\pm0.0034$                 & d & Ama21 \\ 
\noalign{\smallskip}
J21474+627   & TYC 4266-00736-1       &  57 &   0 & $0.606\pm0.020$ & b & $3.64^{+0.50}_{-0.51}$  & $10.8\pm1.5$           & $18.85019\pm0.00013$              & f & Esp22 \\ %Releasing 53 obs  
\noalign{\smallskip}
J22137$-$176 & GJ 1265                &  87 &  11 & $0.178\pm0.018$ & b & $9.82^{+0.51}_{-0.52}$  & $7.4\pm0.5$            & $3.6511\pm0.0001$                 & d & Luq18 \\
\noalign{\smallskip}
J22252+594   & GJ 4276                & 100 &   0 & $0.406\pm0.030$ & b & $8.79\pm0.27$           & $16.57^{+0.94}_{-0.95}$& $13.352\pm0.003$                  & d & Nag19 \\
\noalign{\smallskip}
J22532$-$142 & GJ 876                 &  28 & 594 & $0.350\pm0.013$ & b & $212.07^{+0.27}_{-0.26}$& $760.9^{+1.0}_{-1.0}$  & $61.082^{+0.006}_{-0.010}$        & r & Tri18 \\ %Releasing 69 obs
             &                        &     &     &                 & c & $88.34^{+0.23}_{-0.25}$ & $241.5^{+0.7}_{-0.6}$  & $30.126^{+0.011}_{-0.003}$        & r & Tri18 \\ %Releasing 69 obs
             &                        &     &     &                 & d & $6.14^{+0.23}_{-0.22}$  & $6.91^{+0.22}_{-0.27}$ & $1.938^{+0.001}_{-0.001}$         & r & Tri18 \\ %Releasing 69 obs
             &                        &     &     &                 & e & $3.39^{+0.29}_{-0.28}$  & $15.4\pm1.3$           & $124.4^{+0.3}_{-0.7}$             & r & Tri18 \\ %Releasing 69 obs

==> Tab/occurrence_signals.tex <==
J00051+457 & ~ & ~ & no signal \\      
J00067-075 & ~ & ~ & no signal \\      
J00162+198E & ~ & ~ & no signal \\      
J00183+440$^1$ & 40.68 & 0.0912\% &  rotation\\   
J00184+440 &10136.69 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J00286-066 & ~ & ~ & no signal \\      
J00389+306 &20.17 & 0.0203\% &  unsolved \\    
J00570+450 & ~ & ~ & no signal \\      
J01013+613 & ~ & ~ & no signal \\      
J01025+716 &43.53 & $ < 10^{-6} $ &  dLW \\    
J01026+623$^1$ & 18.9 & 0.0359\% &   H$\alpha$ \\  
J01026+623$^1$ & 9.35 & 0.0036\% &  rotation \\   
J01048-181 & ~ & ~ & no signal \\      
J01125-169$^1$ &3.06 & 0.0108\%  &  known planet \\   
J01125-169$^1$ &4.7 & 0.0346\%  &  known planet \\   
J01125-169$^1$ &80.77 & 0.0004\% &   dLW \\  
J01339-176 & ~ & ~ & no signal \\      
J01433+043 & ~ & ~ & no signal \\      
J01518+644 & ~ & ~ & no signal \\      
J02002+130 &1.95 & $ < 10^{-6} $ &   H$\alpha$, CRX, dLW \\
J02002+130 &782.52 & $ < 10^{-6} $ &  known planet \\    
J02015+637 & ~ & ~ & no signal \\      
J02070+496 & ~ & ~ & no signal \\      
J02123+035 & ~ & ~ & no signal \\      
J02222+478$^4$ &28.29 & 0.0048\% &   dLW \\  
J02336+249 & ~ & ~ & no signal \\      
J02358+202 & ~ & ~ & no signal \\      
J02362+068 & ~ & ~ & no signal \\      
J02442+255 & ~ & ~ & no signal \\      
J02530+168 &11.41 & $ < 10^{-6} $  &  known planet \\   
J02530+168 &174.09 & $ < 10^{-6} $ &   CRX \\  
J02530+168 &4.91 & $ < 10^{-6} $  &  known planet \\   
J02565+554W & ~ & ~ & no signal \\      
J03133+047 &2.29 & $ < 10^{-6} $  &  known planet \\   
J03133+047 &67.52 & 0.2525\%  &  rotation \\   
J03181+382 & ~ & ~ & no signal \\      
J03213+799 & ~ & ~ & no signal \\      
J03217-066 & ~ & ~ & no signal \\      
J03463+262 & ~ & ~ & no signal \\      
J03531+625 & ~ & ~ & no signal \\      
J04153-076 &1.8 & $ < 10^{-6} $ &   CRX \\  
J04225+105 & ~ & ~ & no signal \\      
J04290+219 &12.54 & 0.0036\% &  rotation \\   
J04290+219 &170.18 & 0.0489\% &  CRX \\    
J04290+219 &24.99 & 0.0326\% &   H$\alpha$, dLW \\ 
J04376-110 & ~ & ~ & no signal \\      
J04376+528 &16.32 & 0.3865\% &   H$\alpha$, dLW \\ 
J04376+528 &419.62 & 0.7739\% &   CaIRT \\  
J04376+528 &7.9 & 0.3618\% &  unsolved \\    
J04429+189$^3$ & ~ & ~ & no signal \\      
J04429+214 & ~ & ~ & no signal \\      
J04520+064$^2$ &10582.5 & 0.1972\% &  $P$ > $\frac{2}{3}$ time baseline \\
J04538-177$^1$ $^3$ & ~ & ~ & no signal \\      
J04588+498 &8.89 & 0.0140\% &  unsolved \\    
J05033-173 &1.92 & 0.0015\% &  candidate \\    
J05033-173 &73.78 & 0.4055\% &  unsolved \\    
J05127+196 & ~ & ~ & no signal \\      
J05280+096 & ~ & ~ & no signal \\      
J05314-036 &1362.47 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J05314-036 &34.09 & 0.0022\% &   H$\alpha$ \\  
J05348+138 & ~ & ~ & no signal \\      
J05360-076 & ~ & ~ & no signal \\      
J05365+113 &11.76 & $ < 10^{-6} $ &   H$\alpha$, dLW \\ 
J05365+113 &12.45 & 0.0043\% &   H$\alpha$, dLW \\ 
J05365+113 &6.31 & 0.0836\% &  activity \\    
J05366+112 & ~ & ~ & no signal \\      
J05415+534 &9.03 & 0.0070\% &   CaIRT \\  
J05421+124 & ~ & ~ & no signal \\      
J06011+595 &44.0 & 0.0268\% &  dLW \\    
J06011+595 &82.97 & 0.0821\% &   dLW \\  
J06024+498 & ~ & ~ & no signal \\      
J06103+821 &409.8 & 0.0081\% &   CaIRT \\  
J06105-218 &2621.33 & 0.0001\% &  $P$ > $\frac{2}{3}$ time baseline \\
J06371+175$^1$ & ~ & ~ & no signal \\      
J06421+035 & ~ & ~ & no signal \\      
J06548+332 &120.37 & $ < 10^{-6} $  &  rotation \\   
J06548+332 &14.24 & $ < 10^{-6} $  &  known planet \\   
J06548+332 &53.65 & 0.0024\%  &  rotation \\   
J06594+193 & ~ & ~ & no signal \\      
J07033+346 & ~ & ~ & no signal \\      
J07044+682 & ~ & ~ & no signal \\      
J07274+052 &19.62 & 0.0813\% &  known planet \\    
J07274+052 &461.91 & $ < 10^{-6} $ &  unsolved \\    
J07274+052 &95.0 & $ < 10^{-6} $ &  rotation \\   
J07287-032 &616.27 & 0.5847\% &  unsolved \\    
J07319+362N &4.78 & 0.6855\% &  unsolved \\    
J07393+021 &29.78 & 0.0121\% &  activity \\    
J07403-174 &6.61 & 0.1475\% &  unsolved \\    
J07582+413 & ~ & ~ & no signal \\      
J08119+087 & ~ & ~ & no signal \\      
J08126-215 & ~ & ~ & no signal \\      
J08161+013 &22.45 & 0.1773\% &  rotation \\   
J08293+039 & ~ & ~ & no signal \\      
J08315+730 & ~ & ~ & no signal \\      
J08358+680 &1.73 & 0.1084\% &  unsolved \\    
J08409-234 &710.89 & $ < 10^{-6} $ &  known planet \\    
J08413+594 &10118.37 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J08413+594 &203.24 & $ < 10^{-6} $  &  known planet \\   
J08413+594 &2204.2 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J08526+283 & ~ & ~ & no signal \\      
J09028+680 & ~ & ~ & no signal \\      
J09143+526 &1210.67 & 0.1987\% &  $P$ > $\frac{2}{3}$ time baseline \\
J09143+526 &16.28 & $ < 10^{-6} $ &   H$\alpha$, dLW \\ 
J09144+526 &16.66 & $ < 10^{-6} $ &   H$\alpha$, dLW \\ 
J09144+526 &24.43 & 0.0003\%  &  known planet \\   
J09144+526 &3971.21 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J09307+003 &294.04 & 0.5392\% &  unsolved \\    
J09360-216$^3$ & ~ & ~ & no signal \\      
J09411+132 & ~ & ~ & no signal \\      
J09423+559 & ~ & ~ & no signal \\      
J09425+700 &677.39 & 0.7290\% &  unsolved \\    
J09428+700 &2.48 & 0.0303\% &   H$\alpha$ \\  
J09447-182 & ~ & ~ & no signal \\      
J09468+760 & ~ & ~ & no signal \\      
J09511-123 & ~ & ~ & no signal \\      
J09561+627$^4$ &18.69 & $ < 10^{-6} $ &   H$\alpha$, dLW \\ 
J10023+480 &3.82 & 0.7102\% &  known planet \\    
J10122-037 &10.66 & 0.0008\% &  rotation \\   
J10122-037 &21.43 & 0.0048\% &   H$\alpha$ \\  
J10167-119 & ~ & ~ & no signal \\      
J10196+198 &2.24 & $ < 10^{-6} $ &   CRX \\  
J10251-102 & ~ & ~ & no signal \\      
J10289+008$^1$ &317.21 & 0.0051\% &  unsolved \\    
J10350-094 & ~ & ~ & no signal \\      
J10482-113 &1.52 & 0.0415\% &   dLW \\  
J10482-113 &2.93 & 0.1639\% &  rotation \\   
J10508+068 & ~ & ~ & no signal \\      
J10564+070$^4$ &2.7 & $ < 10^{-6} $ &   CRX, dLW \\ 
J10584-107 &1.27 & $ < 10^{-6} $ &   CRX \\  
J11000+228 & ~ & ~ & no signal \\      
J11026+219 &13.76 & 0.0030\% &   CRX \\  
J11026+219 &13.93 & 0.2527\% &   CRX \\  
J11033+359 &12.94 & $ < 10^{-6} $  &  known planet \\   
J11033+359 &2017.54 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J11054+435 &1026.37 & 0.0001\% &  $P$ > $\frac{2}{3}$ time baseline \\
J11055+435 & ~ & ~ & no signal \\      
J11110+304W & ~ & ~ & no signal \\      
J11126+189 & ~ & ~ & no signal \\      
J11306-080 & ~ & ~ & no signal \\      
J11417+427 &45.9 & $ < 10^{-6} $  &  known planet \\   
J11417+427 &639.31 & $ < 10^{-6} $ &   H$\alpha$ \\  
J11417+427 &835.19 & 0.0736\% &  $P$ > $\frac{2}{3}$ time baseline \\
J11421+267 &2.64 & $ < 10^{-6} $  &  known planet \\   
J11467-140 & ~ & ~ & no signal \\      
J11476+786 & ~ & ~ & no signal \\      
J11477+008$^1$ & ~ & ~ & no signal \\      
J11509+483 &316.73 & $ < 10^{-6} $ &  rotation \\   
J11511+352 &11.12 & 0.0014\% &  rotation \\   
J12100-150 & ~ & ~ & no signal \\      
J12111-199 & ~ & ~ & no signal \\      
J12123+544S &13.67 & $ < 10^{-6} $  &  known planet \\   
J12230+640 &15.13 & 0.0005\% &   CRX \\  
J12230+640 &73.06 & 0.0586\% &   CRX \\  
J12230+640 &8254.83 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J12248-182 & ~ & ~ & no signal \\      
J12312+086 & ~ & ~ & no signal \\      
J12373-208 & ~ & ~ & no signal \\      
J12479+097 &1.42 & $ < 10^{-6} $  &  known planet \\   
J12479+097 &650.94 & 0.3179\%  &  unsolved \\   
J13102+477 & ~ & ~ & no signal \\      
J13209+342 &5962.88 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J13229+244 &3.02 & $ < 10^{-6} $  &  known planet \\   
J13229+244 &87.79 & 0.0015\% &   H$\alpha$, CRX, dLW \\
J13299+102$^1$ &15.42 & 0.3861\% &  rotation \\   
J13299+102$^1$ &15.83 & 0.0023\% &  rotation \\   
J13299+102$^1$ &512.48 & 0.0589\% &  unsolved \\    
J13427+332 & ~ & ~ & no signal \\      
J13450+176 & ~ & ~ & no signal \\      
J13457+148 &105.98 & 0.0074\% &  rotation \\   
J13457+148 &306.51 & 0.0020\% &  unsolved \\    
J13457+148 &33.89 & 0.0007\% &  unsolved \\    
J13458-179 & ~ & ~ & no signal \\      
J13582+125 & ~ & ~ & no signal \\      
J14010-026$^3$ & ~ & ~ & no signal \\      
J14082+805 & ~ & ~ & no signal \\      
J14251+518 & ~ & ~ & no signal \\      
J14257+236E & ~ & ~ & no signal \\      
J14257+236W &10002.44 & 0.2462\% &  $P$ > $\frac{2}{3}$ time baseline \\
J14307-086 &252.02 & 0.2434\% &  unsolved \\    
J14342-125 &113.37 & $ < 10^{-6} $ &   CaIRT \\  
J14342-125 &36.11 & 0.0015\% &  known planet \\    
J14524+123 &26.71 & 0.0010\% &  rotation? \\    
J14544+355 & ~ & ~ & no signal \\      
J15013+055 & ~ & ~ & no signal \\      
J15095+031 & ~ & ~ & no signal \\      
J15194-077 &12.92 & 0.0148\%  &  known planet \\   
J15194-077 &5.37 & $ < 10^{-6} $  &  known planet \\   
J15598-082 & ~ & ~ & no signal \\      
J16028+205 & ~ & ~ & no signal \\      
J16167+672N &42.22 & 0.0208\% &  activity \\    
J16167+672S &21.99 & 0.0641\% &   rotation \\  
J16167+672S &365.13 & $ < 10^{-6} $ &   CaIRT, CRX \\ 
J16167+672S &86.43 & $ < 10^{-6} $ &   known planet \\  
J16254+543$^1$ & ~ & ~ & no signal \\      
J16303-126 &1.26 & 0.3514\% &   known planet \\  
J16303-126 &17.88 & $ < 10^{-6} $  &  known planet \\   
J16303-126 &1.84 & 0.3134\%  &  unsolved \\   
J16327+126 & ~ & ~ & no signal \\      
J16462+164 & ~ & ~ & no signal \\      
J16554-083N & ~ & ~ & no signal \\      
J16581+257 &12.42 & 0.0500\% &  rotation \\   
J16581+257$^3$ &661.35 & 0.0033\% &  $P$ > $\frac{2}{3}$ time baseline \\
J17033+514 &6.94 & 0.0752\% &  candidate \\    
J17052-050 & ~ & ~ & no signal \\      
J17071+215 & ~ & ~ & no signal \\      
J17115+384 &5.58 & 0.8902\% &  unsolved \\    
J17166+080 & ~ & ~ & no signal \\      
J17198+417 &23.13 & 0.3605\% &  unsolved \\    
J17303+055 & ~ & ~ & no signal \\      
J17355+616$^3$ & ~ & ~ & no signal \\      
J17364+683 &38.56 & $ < 10^{-6} $ &   known planet \\  
J17378+185 &15.52 & 0.0001\%  &  known planet \\   
J17378+185 &40.28 & 0.4268\% &   H$\alpha$, dLW \\ 
J17378+185 &499.08 & 0.0479\%  &  known planet \\   
J17542+073 &1.55 & 0.2591\% &  activity \\    
J17578+046$^1$ &287.23 & 0.0056\% &  rotation \\   
J17578+046$^1$ &387.44 & 0.2243\% &   CaIRT, H$\alpha$, dLW \\
J17578+046$^1$ &652.12 & 0.0225\% &  unsolved \\    
J17578+465 & ~ & ~ & no signal \\      
J18027+375 & ~ & ~ & no signal \\      
J18051-030 & ~ & ~ & no signal \\      
J18075-159 & ~ & ~ & no signal \\      
J18165+048 &23239.74 & 0.0095\% &  $P$ > $\frac{2}{3}$ time baseline \\
J18174+483 &16.04 & 0.0332\% &  activity \\    
J18174+483 &7.96 & 0.4972\% &   CRX \\  
J18180+387E & ~ & ~ & no signal \\      
J18221+063 & ~ & ~ & no signal \\      
J18224+620 &2.06 & 0.7429\% &   CaIRT \\  
J18319+406 &2.93 & 0.2034\% &  unsolved \\    
J18346+401 &5786.99 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J18353+457$^3$ &2.62 & 0.0842\% &   H$\alpha$ \\  
J18363+136 &8189.81 & 0.9454\% &  $P$ > $\frac{2}{3}$ time baseline \\
J18409-133 &5.1 & 0.2652\% &  candidate \\    
J18419+318 & ~ & ~ & no signal \\      
J18427+596N &11.2 & 0.0018\% &  unsolved \\    
J18427+596N &27647.04 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J18427+596N &64.8 & 0.0871\% &  unsolved \\    
J18427+596S &10000.0 & $ < 10^{-6} $ &  unsolved \\    
J18427+596S &117.9 & 0.0053\% &  unsolved \\    
J18427+596S &186.6 & 0.0209\% &  unsolved \\    
J18480-145 & ~ & ~ & no signal \\      
J18482+076 &1.4 & 0.8063\% &  rotation \\   
J18498-238 &1.43 & 0.0294\% &   CRX, dLW \\ 
J18498-238 &2.89 & $ < 10^{-6} $ &   dLW \\  
J18580+059$^3$ & ~ & ~ & no signal \\      
J19070+208 & ~ & ~ & no signal \\      
J19072+208 & ~ & ~ & no signal \\      
J19084+322 & ~ & ~ & no signal \\      
J19098+176 & ~ & ~ & no signal \\      
J19169+051N$^5$ &132.39 & $ < 10^{-6} $ &   CRX \\  
J19216+208 & ~ & ~ & no signal \\      
J19251+283 & ~ & ~ & no signal \\      
J19346+045 &2.52 & 0.6353\% &  unsolved \\    
J20260+585 &16.21 & 0.0080\% &  known planet \\  
J20260+585 &14.95 & 0.5846\% &  unsolved \\    
J20260+585 &403.71 & $ < 10^{-6} $ &  tellurics \\    
J20305+654 & ~ & ~ & no signal \\      
J20336+617 &175.74 & 0.6727\% &   CRX \\  
J20405+154 &153.66 & 0.7230\% &  unsolved \\    
J20450+444 & ~ & ~ & no signal \\      
J20525-169 & ~ & ~ & no signal \\      
J20533+621 &118.6 & 0.7191\% &   CaIRT, CRX \\ 
J20556-140S & ~ & ~ & no signal \\      
J20567-104 &1.25 & 0.1960\% &  unsolved \\    
J21019-063 & ~ & ~ & no signal \\      
J21152+257 & ~ & ~ & no signal \\      
J21164+025 &14.46 & $ < 10^{-6} $  &  known planet \\   
J21164+025 &43.71 & 0.0006\% &   H$\alpha$ \\  
J21221+229 &39.91 & 0.0001\% &   H$\alpha$, dLW \\ 
J21221+229 &686.81 & $ < 10^{-6} $ &  known planet \\    
J21348+515 &26.33 & 0.7167\% &  rotation \\   
J21463+382 & ~ & ~ & no signal \\      
J21466-001 & ~ & ~ & no signal \\      
J21466+668 &2.31 & $ < 10^{-6} $  &  known planet \\   
J21466+668 &8.05 & 0.0001\%  &  known planet \\   
J21466+668 &92.49 & $ < 10^{-6} $  &  rotation \\   
J22021+014 &10.95 & 0.0373\% &   H$\alpha$ \\  
J22057+656 &122.52 & $ < 10^{-6} $ &   CRX \\  
J22096-046$^2$ &3998.46 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J22114+409 &15.22 & 0.5957\% &  rotation \\   
J22115+184 &374.96 & $ < 10^{-6} $ &   CRX \\  
J22115+184 &39.02 & 0.0015\% &   dLW \\  
J22125+085 &2911.44 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J22137-176 &3.65 & $ < 10^{-6} $  &  known planet \\   
J22137-176 &588.11 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J22231-176 & ~ & ~ & no signal \\      
J22252+594 &13.35 & $ < 10^{-6} $  &  known planet \\   
J22298+414 &5.78 & 0.0280\% &   dLW \\  
J22330+093 &34.06 & 0.6282\% &  unsolved \\    
J22503-070 & ~ & ~ & no signal \\      
J22532-142 &30.07 & $ < 10^{-6} $  &  known planet \\   
J22532-142 &60.85 & $ < 10^{-6} $  &  known planet \\   
J22559+178 & ~ & ~ & no signal \\      
J22565+165 &18.61 & $ < 10^{-6} $ &  rotation \\   
J22565+165 &1845.72 & $ < 10^{-6} $ &  $P$ > $\frac{2}{3}$ time baseline \\
J22565+165 &39.28 & $ < 10^{-6} $ &   H$\alpha$, dLW \\ 
J23216+172 & ~ & ~ & no signal \\      
J23245+578 & ~ & ~ & no signal \\      
J23340+001 & ~ & ~ & no signal \\      
J23351-023 & ~ & ~ & no signal \\      
J23381-162 & ~ & ~ & no signal \\      
J23419+441 &175.09 & 0.0001\% &  unsolved \\    
J23431+365 & ~ & ~ & no signal \\      
J23492+024 &372.77 & 0.0001\% &   CaIRT \\  
J23492+024 &53.83 & 0.4878\% &   H$\alpha$ \\  
J23505-095 & ~ & ~ & no signal \\  
